Quickest Detection of COVID-19 Pandemic Onset

This paper develops an easily-implementable version of Page's CUSUM quickest-detection test, designed to work in certain composite hypothesis scenarios with time-varying data statistics. The decision statistic can be cast in a recursive form and is particularly suited for on-line analysis. By back-testing our approach on publicly-available COVID-19 data we find reliable early warning of infection flare-ups, in fact sufficiently early that the tool may be of use to decision-makers on the timing of restrictive measures that may in the future need to be taken.

==> figures/results-letter-v3.tex <==
\newcommand{\commonScale}{.60}

\psfrag{xla}[c][c]	[.75]{	\raisebox{-10mm}{\hspace{0mm}{$\Delta$ [days]}}}
\psfrag{yla}[c][c]	[.75]{	\raisebox{14mm}{\hspace{0mm}{$R$}}}
%
%
\psfrag{leg1}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Scen. 0, $\alpha/\sigma = 0.5$}}}
\psfrag{leg2}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Scen. 0, $\alpha/\sigma = 0.5$}}}
\psfrag{leg3}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Scen. 1, $\alpha/\sigma = 0.5$}}}
\psfrag{leg4}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Scen. 1, $\alpha/\sigma = 0.5$}}}
\psfrag{leg5}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Scen. 1, $\alpha/\sigma = 1$}}}
\psfrag{leg6}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Scen. 1, $\alpha/\sigma = 1$}}}
\psfrag{leg7}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Scen. 2, $\alpha/\sigma = 0.5$}}}
\psfrag{leg8}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Scen. 2, $\alpha/\sigma = 0.5$}}}
\psfrag{leg9}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{MAST - Scen. 2, $\alpha/\sigma = 1$}}}
\psfrag{leg10}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Page - Scen. 2, $\alpha/\sigma = 1$}}}
%
%
\newcommand{\xscale}{.75}
\newcommand{\xhoff}{\hspace{-1mm}}
\newcommand{\xvoff}{\raisebox{-6mm}}
%
\psfrag{x1}[c][c]	[\xscale]{	\xvoff{\xhoff $0$}}
\psfrag{x2}[c][c]	[\xscale]{	\xvoff{\xhoff $5$}}
\psfrag{x3}[c][c]	[\xscale]{	\xvoff{\xhoff $10$}}
\psfrag{x4}[c][c]	[\xscale]{	\xvoff{\xhoff $15$}}
\psfrag{x5}[c][c]	[\xscale]{	\xvoff{\xhoff $20$}}
\psfrag{x6}[c][c]	[\xscale]{	\xvoff{\xhoff $25$}}
\psfrag{x7}[c][c]	[\xscale]{	\xvoff{\xhoff $30$}}
%
%
\newcommand{\yscale}{.75}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y1}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-9}$}}
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-8}$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-7}$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-6}$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-5}$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-4}$}}
\psfrag{y7}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-3}$}}
\psfrag{y8}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-2}$}}
\psfrag{y9}[r][r]	[\yscale]{	\yvoff{\yhoff $10^{-1}$}}
\psfrag{y10}[r][r]	[\yscale]{	\yvoff{\yhoff $1$}}

==> figures/us-states-MAST.tex <==
\newcommand{\commonScale}{.60}

\psfrag{xla}[c][c]	[.75]{	\raisebox{-12mm}{\hspace{0mm}{Stopping Day}}}
\psfrag{yla}[c][c]	[.75]{	\raisebox{11mm}{\hspace{0mm}{MAST}}}
%
%
\psfrag{leg1}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{California}}}
\psfrag{leg2}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Florida}}}
\psfrag{leg3}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Illinois}}}
\psfrag{leg4}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Ohio}}}
\psfrag{leg5}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{North Carolina}}}
\psfrag{leg6}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Michigan}}}
\psfrag{leg7}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Arizona}}}
\psfrag{leg8}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Massachusetts}}}
\psfrag{leg9}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Indiana}}}
\psfrag{leg10}[lc][lb]	[\commonScale]{	\raisebox{2mm}{\hspace{-1mm}{Tennessee}}}
%
%
\newcommand{\xscale}{.75}
\newcommand{\xhoff}{\hspace{-1mm}}
\newcommand{\xvoff}{\raisebox{-6mm}}
%
\psfrag{x1}[c][c]	[\xscale]{	\xvoff{\xhoff May}}
\psfrag{x2}[c][c]	[\xscale]{	\xvoff{\xhoff Jun}}
\psfrag{x3}[c][c]	[\xscale]{	\xvoff{\xhoff Jul}}
\psfrag{x4}[c][c]	[\xscale]{	\xvoff{\xhoff Aug}}
\psfrag{x5}[c][c]	[\xscale]{	\xvoff{\xhoff Sep}}
\psfrag{x6}[c][c]	[\xscale]{	\xvoff{\xhoff Oct}}
\psfrag{x7}[c][c]	[\xscale]{	\xvoff{\xhoff Nov}}
\psfrag{x8}[c][c]	[\xscale]{	\xvoff{\xhoff Dec}}
\psfrag{year}[c][c]	[\xscale]{	\raisebox{-10mm}{\xhoff 2020}}
%
%
\newcommand{\yscale}{.75}
\newcommand{\yhoff}{\hspace{0mm}}
\newcommand{\yvoff}{\raisebox{0mm}}
%
\psfrag{y2}[r][r]	[\yscale]{	\yvoff{\yhoff $50$}}
\psfrag{y3}[r][r]	[\yscale]{	\yvoff{\yhoff $100$}}
\psfrag{y4}[r][r]	[\yscale]{	\yvoff{\yhoff $150$}}
\psfrag{y5}[r][r]	[\yscale]{	\yvoff{\yhoff $200$}}
\psfrag{y6}[r][r]	[\yscale]{	\yvoff{\yhoff $250$}}
%
%
\psfrag{min}[lc][lb]	[.50]{	\raisebox{8mm}{\hspace{-4mm}{Smallest Thr.}}}
\psfrag{max}[lc][lb]	[.50]{	\raisebox{2mm}{\hspace{-4mm}{Largest Thr.}}}
